INSPECT: A Multimodal Dataset for Pulmonary Embolism Diagnosis and Prognosis

Synthesizing information from multiple data sources plays a crucial role in the practice of modern medicine. Current applications of artificial intelligence in medicine often focus on single-modality data due to a lack of publicly available, multimodal medical datasets. To address this limitation, we introduce INSPECT, which contains de-identified longitudinal records from a large cohort of patients at risk for pulmonary embolism (PE), along with ground truth labels for multiple outcomes. INSPECT contains data from 19,402 patients, including CT images, radiology report impression sections, and structured electronic health record (EHR) data (i.e. demographics, diagnoses, procedures, vitals, and medications). Using INSPECT, we develop and release a benchmark for evaluating several baseline modeling approaches on a variety of important PE related tasks. We evaluate image-only, EHR-only, and multimodal fusion models. Trained models and the de-identified dataset are made available for non-commercial use under a data use agreement. To the best of our knowledge, INSPECT is the largest multimodal dataset integrating 3D medical imaging and EHR for reproducible methods evaluation and research.

==> sections/_1_introduction.tex <==
\section{Introduction}
\label{sec:introduction}
\vspace{-4mm}
%Pulmonary embolism (PE) is a leading cause of death with approximately 100,000 to 200,000 deaths in the United States each year \cite{farmakis2022mortality}. In addition to high risk of mortality, short and long term complications of PE includes PE recurrence, chronic thromboembolic pulmonary hypertension, and bleeding from anticoagulation therapy, causing significant disability. Existing clinical scoring system,  such as Pulmonary Embolism Severity Index (PESI) ~\cite{aujesky2005derivation}, relay heavily on antiquated, rule-based metrics from clinical history and vital signs. When PE is suspected clinically, CTPA is conducted on almost all patients without contraindication, and provides a definite diagnosis of PE. More evidence suggest that imaging biomarkers from CT pulmonart angiogram (CTPA) improve predictive value for adverse events in patients with PE. Having a prediction model that incorporates a multimodality approach, with structured and unstructured clinical data from EHR and imaging data from CTPA would be extremely helpful for clinical risk stratification. 

The synthesis of information from multiple data sources is integral to the practice of modern medicine. This is particularly true for estimating patient long-term outcome and treatment planning, where physicians frequently rely on pertinent and accurate information regarding the current symptoms and past medical history sourced from a wide range of modalities, including imaging, laboratory test results, patient timelines, and medical reports~\cite{leslie2000influence, cohen2007accuracy}.

%Despite the increasingly large effort of using machine learning for healthcare, the performance of artificial intelligence models have been suboptimal for aiding clinical decision making and ultimately improving healthcare planning and patient outcomes. We posit the difficulty lies in the lack of large-scale multi-modal datasets that are publicly available from a wide range of data sources and both carefully curated and readily deployable for machine learning research.
%Physicians use information regarding the current symptoms and past medical history from a wide range of modalities, including imaging, laboratory test results, patient past history, and medical reports to make these assessments~\cite{leslie2000influence, cohen2007accuracy}. 

The accelerated advancements in artificial intelligence (AI) herald the prospect of more efficient and effective diagnostic, prognostic, and treatment planning processes. This evolution carries the potential to significantly enhance healthcare delivery and patient outcomes. However, the majority of current medical AI models only utilize one single modality to inform predictions~\cite{huang2020fusion}, which is in contrast to the present paradigm of practicing medicine~\cite{comfere2014provider, comfere2015dermatopathologists, jonas2018glaucoma}. The lack of medical AI models that synthesize information from multiple modalities is largely due to the constraints of publicly available medical datasets. Many current medical datasets suffer from one of the following limitations: 1) insufficient scale \cite{zhi2022multimodal}, 2) limited multimodality \cite{li2020behrt}, or 3) limited diagnosis and prognosis labels \cite{kumar2022mortality}. Thus, addressing these limitations in publicly available datasets is essential for the further advancement of AI-driven diagnostic and prognostic tools in the medical field.


To help address these challenges, we introduce \dataset~(\textbf{I}ntegrated \textbf{M}ultimodal \textbf{P}rognostic \textbf{E}valuation of \textbf{C}linical \textbf{T}imelines), a large-scale, multimodal dataset of patients at risk for pulmonary embolisms (PE). 
% THis sentence need rework
%We opted to concentrate on PE due to it's numerous known complications that require multimodal approaches to predict
%In addition to high risk of mortality, short and long term complications of PE includes PE recurrence, chronic thromboembolic pulmonary hypertension, and bleeding from anticoagulation therapy, causing significant disability. Existing clinical scoring system,  such as Pulmonary Embolism Severity Index (PESI) ~\cite{aujesky2005derivation}, relay heavily on antiquated, rule-based metrics from clinical history and vital signs. When PE is suspected clinically, CTPA is conducted on almost all patients without contraindication, and provides a definite diagnosis of PE.
We opted to concentrate on PE given its correlation with various intricate outcomes, including high risk of mortality, short and long term complications of PE includes PE recurrence, chronic thromboembolic pulmonary hypertension, and bleeding from anticoagulation therapy, causing significant disability. Moreover, evidence suggest that imaging biomarkers from CT pulmonart angiogram (CTPA) improve predictive value for adverse events in patients with PE~\cite{meinel2015predictive}. Having a prediction model that incorporates a multimodality approach, with structured and unstructured clinical data from EHR and imaging data from CTPA would be extremely helpful for clinical risk. With \dataset, our objective is to expedite the recognition and treatment of PE by delivering a rich, multimodal dataset. Additionally, we offer an array of meticulously curated labels for predicting PE patient outcomes, aspiring to assist hospitals in effective resource management, leading to improved patient care. Our main contributions are as follows: 

%specifically those who have undergone a Computed Tomography Pulmonary Angiogram (CTPA) for PE detection. 
%Our choice of focusing on PE is underscored by both clinical evidence~\cite{banerjee2019comparative} and AI applications~\cite{huang2020multimodal} demonstrating the significance of synthesizing information from multiple medical sources, and incorporating patient medical history, for effective PE diagnosis. Furthermore, prognostic capabilities—predicting mortality and readmission rates for PE patients permit hospitals to strategically distribute resources, thereby enhancing patient outcomes. Conventional strategies, such as the Pulmonary Embolism Severity Index (PESI) scoring system~\cite{aujesky2005derivation}, depend heavily on antiquated, rule-based metrics, neglecting comprehensive data inputs such as CTPA. With \dataset, our objective is to expedite the recognition and treatment of PE by delivering a rich, multimodal dataset. Additionally, we offer an array of meticulously curated labels for predicting PE patient outcomes, aspiring to assist hospitals in effective resource management, leading to improved patient care. Our main contributions are as follows: 


%To help address these challenges, we present \dataset, a large-scale multimodal and multi-label dataset and benchmark. For this multimodal dataset we curate labels for a set of patients susceptible to pulmonary embolisms (PE), a life-threatening medical condition with an estimated 180,000 deaths per year in the United States. Medically it has been known that one single modality of data can not capture the comprehensive view of patients' pathology suffering from this disease \cite{banerjee2019comparative}. Furthermore, estimating PE patient outcomes, including mortality and readmission can hospitals better prepare resources to treating patients, leading to better outcomes. However, current approaches rely on outdated, rule-based metrics such as the Pulmonary Embolism Severity Index (PESI) scoring system~\cite{aujesky2005derivation}. We create this multimodal dataset with the hope to improve rapid recognition and treatment of PE. Furthermore, we curate a set of labels for estimating PE patient outcomes, including mortality and readmission, which can help hospitals better prepare resources for treating patients and lead to better outcomes. Our main contributions are as follows: 

\textbf{1. A large-scale, multimodal medical dataset.} \dataset~contains \ncases~CTPA studies from \npatients~patients, each including: (1) high-resolution CT images (3D volumetric pixel data) with (2) paired radiology reports; and (3) structured electronic health record (EHR) data. Patient EHRs are longitudinal timelines of timestamped medical codes that capture demographics, medications, labs, vitals, procedures and past diagnosis for all prior patient visits. To our knowledge, this is the first dataset to provide 3D medical imaging linked to both radiology reports and longitudinal EHR data.
%, providing significantly more patient history than datasets such as MIMIC-IV~\cite{goldberger2000physiobank,johnson2020mimic}. 

\textbf{2. A benchmark for PE diagnosis and prognosis.} Using our dataset, we develop a benchmark that constructs and evaluates eight clinically important pulmonary embolism tasks using several baseline imaging and EHR modeling approaches.  We evaluate both unimodal models that only use medical images or structured patient EHR data as well as combined fusion models that incorporate information from both images and EHR data. 
%We open-source all the models that we have trained and provide a link to our codebase to ensure reproducibility. 

%ur baseline results indicate that the combination of medical images with electronic health records (EHR) yields the most favorable outcomes in the diagnosis of pulmonary embolism (PE), but not for outcome prediction. This is in contrast to what we expect in the clincal setting where valuable predictive information regarding outcomes, such as the severity of the condition, the likelihood of developing PE, and the treatability of associated conditions like pulmonary hypertension (PH), resides within the pixel data. However, our current simple fusion methods fall short of fully harnessing this potential. Therefore, we have released \dataset to foster the discovery and development of advanced techniques that effectively integrate pixel data and EHR, thereby enabling more accurate outcome prediction in the context of PE.


%\dataset~aims to advance research into multimodal fusion strategies for integrating large-scale 3D medical imaging data and patient EHR data.
%In summary, we introduce a large-scale medical dataset with multiple modalities, outcome labels, and benchmark results.


We share data and pretrained models under Data Use Agreement (DUA) for non-commercial, research use and open source all experimental software.

\begin{figure*}
\begin{center}
\includegraphics[width=1.0\textwidth]{figures/main_figure.png}
\end{center}\vspace{-0.05in}
   \caption{An overview of the \dataset~dataset} 
\label{fig:dataset}\vspace{-0.1in}
\end{figure*}
%The scale of a dataset is crucial for the success of deep learning models, as these models require vast quantities of data for effective training and diverse samples for reliable evaluation. Additionally, multimodality is particularly important in radiology, as accurate diagnostic outcomes often depend on the integration of imaging data with patient health records. Lastly, outcome labels are vital for assessing the performance and capabilities of AI models in diagnostic and prognostic tasks. Thus, addressing these limitations in publicly available datasets is essential for the further advancement of AI-driven diagnostic and prognostic tools in the medical field.


% The synthesis of information from multiple data sources is integral to the practice of modern medicine. This is particularly true for estimating patient long-term outcome prognosis and treatment planning, where physicians frequently rely on pertinent and accurate information regarding the current symptoms and past medical history sourced from a wide range of modalities, including imaging, laboratory test results, patient timelines, and medical reports. Several studies have shown that the lack of access to these relevant clinical data can negatively affect a physician's performance and ultimately limit patient outcomes~\cite{leslie2000influence, cohen2007accuracy}. 

% The rapid progress in artificial intelligence (AI) has opened the door to the potential for automating diagnosis, prognosis, and treatment planning, ultimately improving healthcare and patient outcomes. However, the majority of current medical AI models only utilize only a single modality to inform predictions~\cite{huang2020fusion}, which is in contrast to the present paradigm of practicing medicine~\cite{comfere2014provider, comfere2015dermatopathologists, jonas2018glaucoma}. The lack of medical AI models that synthesize information from multiple modalities is largely due to the constraints of publicly available medical datasets. Many current medical datasets suffer from one of the following limitations: 1) insufficient scale, 2) limited multimodality, or 3) limited diagnosis and prognosis labels. Thus, addressing these limitations in publicly available datasets is essential for the further advancement of AI-driven diagnostic and prognostic tools in the medical field.

% To help address these challenges, we present \dataset, a large-scale multimodal and multi-label dataset and benchmark. We focus on patients susceptible to pulmonary embolisms, a life-threatening medical condition with an estimated 180,000 deaths per year in the United States, as we believe PE is an area where AI can make a significant contributions. Specifically, rapid recognition and treatment of PE have been shown to significantly reduce the mortality rate of PE, yet diagnosis of PE is often delayed. Furthermore, estimating PE patient outcomes, including mortality and readmission can hospitals better prepare resources to treating patients, leading to better outcomes. Yet current approaches rely on outdated, rule-based metrics such as the Pulmonary Embolism Severity Index (PESI) scoring system~\cite{aujesky2005derivation}.
% Our main contributions are as follows: 

% \textbf{1. A large-scale medical dataset with multiple modalities.} \dataset~contains a total of \ncases~cases from \npatients~patients, each including high-quality CT images (3D volumetric pixel data), accompanying radiology reports, and patient electronic health records (EHR) data. Patient EHRs are represented as timelines of timestamped, medical codes. These longitudinal data includes patient demographics, medications, lab results, vitals, procedures and past diagnosis for all prior patient visits, providing significantly more patient history than datasets such as MIMIC-VI. 

% \textbf{2. Multiple diagnostic and prognosis labels.} \dataset~includes a diagnostic label for identifying patients with pulmonary embolisms and 3 prognosis labels (i.e., future patient outcomes) for in-hospital mortality, re-admission, and pulmonary hypertension (PH) at varying 1 to 12 month time horizons. 
% These labels are derived either from the patient's EHR or evidence from clinical notes, identified using natural language processing (NLP) labelers trained on clinician annotated notes. To ensure reproducibility, we describe in detail the steps we take to derive these labels and open-source our NLP labelers. 

% \textbf{3. A benchmark for PE diagnosis and prognosis for subsequent outcomes.} In addition to the data and labels, we develop and evaluate baseline predictive models for each of the tasks outlined in this paper. We not only provide single-modality models that use only medical images, reports, or patient EHR for each task but also experiment with simple fusion strategies. 
% %We open-source all the models that we have trained and provide a link to our codebase to ensure reproducibility. 

% \dataset~aims to advance research into multimodal fusion strategies for integrating large-scale 3D medical imaging data and patient EHR data.
% %In summary, we introduce a large-scale medical dataset with multiple modalities, outcome labels, and benchmark results.
% We share all data and pretrained models under Data Use Agreement (DUA) for non-commercial, research use and open source all experimental software. 

==> tables/PH_hand_statistics.tex <==
\begin{longtable}{|c|c|c|c|c|}
\caption{Statistics for \textbf{PH mentions} and \textbf{functional measurements} in our labeled data where we separate the data counts by per patient and per note} \label{table:PH_hand_stat} \\ 
\hline
 & \multicolumn{2}{c|}{Validation set} & \multicolumn{2}{c|}{Test set} \\
\hline
\hline
\endfirsthead
PH mention & \# per note & \# per patient & \# per note & \# per patient  \\ 
\hline
Historical Positive & 54 & 18 & 59 & 30 \\
Hypothetical & 6 & 5 & 4 & 3 \\
N/A & 121 & 32 & 122 & 52 \\
Negative & 1 & 1 & 1 & 1 \\
Negative Hedged & 4 & 4 & 3 & 3 \\
Other Meaning & 28 & 14 & 36 & 22 \\
Positive & 106 & 29 & 123 & 45 \\
Positive Hedged & 30 & 18 & 33 & 22 \\
Unclear & 19 & 11 & 23 & 18 \\
\hline
Functional measurement & \# per note & \# per patient & \# per note & \# per patient  \\ 
\hline
+RV Dysfunction & 86 & 21 & 84 & 30 \\
-RV Dysfunction & 24 & 13 & 20 & 14 \\
N/A & 114 & 30 & 150 & 57 \\
PAP <25 & 7 & 4 & 0 & 0 \\
PAP $\ge$25 & 32 & 10 & 24 & 11 \\
RVSP >45 & 95 & 24 & 128 & 44 \\
RVSP $\le$45 & 48 & 23 & 26 & 21 \\
\hline
\multicolumn{5}{|c|}{Synthetized labels for current PH and historical PH} \\
\hline
Current PH Negative & 5 & 5 & 4 & 4 \\
Current PH Positive & 121 & 33 & 142 & 53 \\
Current PH Unknown & 143 & 38 & 169 & 63 \\
\hline
Historical PH Positive & 54 & 18 & 59 & 30 \\
Historical PH Unknown & 170 & 41 & 191 & 66 \\
\hline
\end{longtable}

==> tables/hand_label_table.tex <==
\begin{table}[h]
\centering

\begin{tabular}{cccc}
\toprule

\textbf{Label Type} & \textbf{\# Labels} & \textbf{\# Positive} & \textbf{\# Negative} \\
\midrule

Pulmonary Embolism & 4,351 & 1,424 & 2,927 \\ 

Pulmonary Hypertension &  &  &  \\ 

\bottomrule

\end{tabular}

\vspace{0.2in}
\caption{Statistics for the manual expert radiologist labels in our dataset. }
\label{table:hand_label}
\end{table}





==> tables/main_table.tex <==
\begin{table}[h]
\centering
\caption{Summary of Dataset}
\begin{tabular}{cc|c|c|c|c}
\toprule
\multicolumn{6}{c}{\textbf{Demographics Statistics}} \\
\midrule
%$\rowcolor{lightgray}
\textbf{Attributes} &  & \multicolumn{1}{c|}{\textbf{All}} & \multicolumn{1}{c|}{\textbf{Train}} & \multicolumn{1}{c|}{\textbf{Val}} & \multicolumn{1}{c}{\textbf{Test}} \\
\midrule
%& & \textbf{count} & \textbf{\%} & \textbf{count} & \textbf{\%} & \textbf{count} & \textbf{\%} & \textbf{count} & \textbf{\%} \\
%\midrule
\midrule

%\rowcolor{lightgray}
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{}}} 
& Cases & -- & -- & -- & -- \\
& Patients & -- & -- & -- & -- \\

%\midrule

\multirow{3}{*}{\textbf{Gender}}
& Female    & -- & -- & -- & -- \\
& Male      & -- & -- & -- & -- \\
& Unknown   & -- & -- & -- & -- \\
\midrule
\multirow{3}{*}{\textbf{Age}}
& 0-20      & -- & -- & -- & -- \\
& 21-40     & -- & -- & -- & -- \\
& 41-60     & -- & -- & -- & -- \\
& 61-80     & -- & -- & -- & -- \\
& 81+       & -- & -- & -- & -- \\
& Unknown   & -- & -- & -- & -- \\
\midrule
\multirow{3}{*}{\textbf{Race}}
& White     & -- & -- & -- & -- \\
& Black     & -- & -- & -- & -- \\
& Hispanic  & -- & -- & -- & -- \\
& Asian     & -- & -- & -- & -- \\
& Native    & -- & -- & -- & -- \\
& Other     & -- & -- & -- & -- \\
& Unknown   & -- & -- & -- & -- \\
\midrule
\midrule
\multicolumn{6}{c}{\textbf{Labels Statistics}} \\
\midrule
%\midrule
\multirow{3}{*}{\textbf{Pulmonary Embolism}}
& Positive  & -- & -- & -- & -- \\
& Negative  & -- & -- & -- & -- \\
\midrule
\multirow{3}{*}{\textbf{Mortality}}
& 30 day    & -- & -- & -- & -- \\
& 6 months  & -- & -- & -- & -- \\
& 1 year    & -- & -- & -- & -- \\
\midrule
\multirow{3}{*}{\textbf{Re-admission}}
& 30 day    & -- & -- & -- & -- \\
& 6 months  & -- & -- & -- & -- \\
& 1 year    & -- & -- & -- & -- \\
\midrule
\multirow{1}{*}{\textbf{Pulmonary Hypertension}}
& 1 year    & -- & -- & -- & -- \\
\bottomrule

\end{tabular}
\label{table:1}
\end{table}

\caption{Summary statistics of the \dataset dataset for all, training, validation, and test sets. The table provides a comprehensive overview of patient demographics, clinical characteristics, and outcomes. Categories include overall case and patient count, detailed demographic distribution, and specific diagnostic and prognostic labels.}

==> tables/nlp_pe_performance.tex <==
\begin{table}
\centering
\scalebox{0.7}{
\begin{tabular}{c|c|c|c}
\toprule
      & Positive PE & Subsegmental PE & Acute PE \\
\hline
AUROC     & 0.99 & 0.99 & 0.99 \\
F1        & 0.97 & 0.95 & 0.96 \\
Precision & 0.97 & 0.98 & 0.98 \\
Recall    & 0.98 & 0.93 & 0.94 \\


\bottomrule
\end{tabular}
}

\vspace{0.2in}
\caption{NLP PE labeler performance}
\label{table:nlp_pe}
\vspace{-0.1in}
\end{table}
